Efficient Fuzz Testing for Apache Spark Using Framework Abstraction

The emerging data-intensive applications are increasingly dependent on data-intensive scalable computing (DISC) systems, such as Apache Spark, to process large data. Despite their popularity, DISC applications are hard to test. In recent years, fuzz testing has been remarkably successful; however, it is nontrivial to apply such traditional fuzzing to big data analytics directly because: (1) the long latency of DISC systems prohibits the applicability of fuzzing, and (2) conventional branch coverage is unlikely to identify application logic from the DISC framework implementation. We devise a novel fuzz testing tool called BigFuzz that automatically generates concrete data for an input Apache Spark program. The key essence of our approach is that we abstract the dataflow behavior of the DISC framework with executable specifications and we design schema-aware mutations based on common error types in DISC applications. Our experiments show that compared to random fuzzing, BigFuzz is able to speed up the fuzzing time by 1477X, improves application code coverage by 271%, and achieves 157% improvement in detecting application errors. The demonstration video of BigFuzz is available at https://www.youtube.com/watch?v=YvYQISILQHs&feature=youtu.be.

==> data.tex <==
\tool is available at \url{https://github.com/qianzhanghk/BigFuzz}, and the demonstration video of \tool is available at \url{\footnotesize https://www.youtube.com/watch?v=YvYQISILQHs&feature=youtu.be}.


==> plots/cov/P1.tex <==

 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,33.33)
        (100, 66.67)
        (200,100)
        (500, 100)
        (1000,100)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,44.40)
            (100,55.50)
            (200,77.70)
            (500,83.5)
            (1000, 89)
    };
    

==> plots/cov/P2.tex <==

 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,40.91)
        (100, 72.73)
        (200,72.73)
        (500, 86.36)
        (1000, 86.36)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,50)
            (100,56.25)
            (200,68.75)
            (500,75)
            (1000, 75)
    };
    

==> plots/cov/P3.tex <==


 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,42.80)
        (100, 75)
        (200,75)
        (500, 92.80)
        (1000, 100)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,10.91)
            (100,72.73)
            (200,83)
            (500,86.36)
            (1000, 100)
    };
    

==> plots/cov/P4.tex <==
%	68.19%	72.73%	81.30%	85.00%

 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,40.91)
        (100, 68.19)
        (200,72.73)
        (500, 100)
        (1000, 100)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,44.40)
            (100,44.40)
            (200,65)
            (500,83.5)
            (1000, 89)
    };


==> plots/cov/P5.tex <==
 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,54.16)
        (100, 83.33)
        (200,93.33)
        (500, 93.33)
        (1000, 93.33)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,33.33)
            (100,58.33)
            (200,62.5)
            (500,83.33)
            (1000, 91.67)
    };
    

==> plots/cov/P6.tex <==
 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,5.00)
        (100, 10.91)
        (200,25)
        (500, 37)
        (1000, 65)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,16.31)
            (100,16.31)
            (200,26.5)
            (500,29.9)
            (1000, 45)
    };
    

==> plots/cov/P7.tex <==
 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,25)
        (100, 25)
        (200,28.125)
        (500, 43.75)
        (1000, 51.25)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,9.23)
            (100,31)
            (200,33.33)
            (500,50.5)
            (1000, 56.67)
    };
    

==> plots/div/P1.tex <==

  \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,0)
        (100, 0.2496)
        (200,0.02496)
        (500, 0.498)
        (1000,1.248)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,2)
            (100,4.98)
            (200,4.98)
            (500,5.748)
            (1000, 5.748)
    };

==> plots/div/P2.tex <==
  
  \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,0)
        (100, 0.2496)
        (200,0.02496)
        (500, 0.498)
        (1000,1.248)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,2.74)
            (100,4.75)
            (200,5.25)
            (500,5.25)
            (1000, 5.25)
    };


==> plots/div/P3.tex <==
  
  \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,0)
        (100, 0)
        (200, 0)
        (500, 0)
        (1000, 0)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,2.25)
            (100,4)
            (200,4.25)
            (500,4.5)
            (1000, 4.5)
    };

==> plots/div/P4.tex <==

  \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,0.982)
        (100, 1.116)
        (200, 1.25)
        (500, 1.875)
        (1000, 1.875)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,2.25)
            (100,2.25)
            (200,4)
            (500,4.25)
            (1000, 4.75)
    };

==> plots/div/P5.tex <==

  \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,0)
        (100, 0.5)
        (200, 1.25)
        (500, 1.25)
        (1000, 1.875)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,1)
            (100,3.5)
            (200,6.25)
            (500,6.5)
            (1000, 7)
    };

==> plots/div/P6.tex <==
    \addplot[smooth, mark=*,red]
    plot coordinates {
            (0,0)
            (10,0.5)
            (100,0.5)
            (200,1.876)
            (500,2)
            (1000,2)
    };
    
\addlegendentry{\tool Divergence} 
    \addplot[smooth, mark=*,blue]
      plot coordinates {
            (0,0)
            (10,3)
            (100,5)
            (200,6)
            (500,6)
            (1000,9)
    };

==> plots/div/P7.tex <==
    \addplot[smooth, mark=*,red]
    plot coordinates {
            (0,0)
            (10,0.25)
            (100,1)
            (200,1)
            (500,1.875)
            (1000,2)
    };
    

    \addplot[smooth, mark=*,blue]
      plot coordinates {
            (0,0)
            (10,5.5)
            (100,5.5)
            (200,6.875)
            (500,9)
            (1000,9)
    };

==> plots/percentage/P1.tex <==

 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,3)
        (100,3.8)
        (200,3.8)
        (500,3.8)
        (1000,4)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,2)
            (100,4.98)
            (200,4.98)
            (500,5.748)
            (1000, 5.748)
    };
    

==> plots/percentage/P2.tex <==

 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,0.75)
        (100,0.75)
        (200,0.75)
        (500,1)
        (1000,1.5)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,2.74)
            (100,4.75)
            (200,5.25)
            (500,5.25)
            (1000, 5.25)
    };


==> plots/percentage/P3.tex <==

 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,0.75)
        (100,1)
        (200,1)
        (500,1)
        (1000,1)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,2.25)
            (100,4)
            (200,4.25)
            (500,4.5)
            (1000, 4.5)
    };

==> plots/percentage/P4.tex <==

 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,1.5)
        (100,2.5)
        (200,2.5)
        (500,2.5)
        (1000,3)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,2.25)
            (100,2.25)
            (200,4)
            (500,4.25)
            (1000, 4.75)
    };

==> plots/percentage/P5.tex <==

 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,0.5)
        (100,1.2)
        (200,1.2)
        (500,1.2)
        (1000,2)
    };

    \addplot[smooth,mark=*,blue] 
        plot coordinates {
            (0,0)
            (10,1)
            (100,3.5)
            (200,6.25)
            (500,6.5)
            (1000, 7)
    };
    

==> plots/percentage/P6.tex <==

 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,1.5)
        (100,2)
        (200,2)
        (500,2)
        (1000,2.75)
    };

\addlegendentry{\tool Divergence} 
    \addplot[smooth, mark=*,blue]
      plot coordinates {
            (0,0)
            (10,3)
            (100,5)
            (200,6)
            (500,6)
            (1000,9)
    };
    

==> plots/percentage/P7.tex <==

 \addplot[smooth,mark=*,red] plot coordinates {
        (0,0)
        (10,1.75)
        (100,1.75)
        (200,2.75)
        (500,4)
        (1000,4.75)
    };

    \addplot[smooth, mark=*,blue]
      plot coordinates {
            (0,0)
            (10,5.5)
            (100,5.5)
            (200,6.875)
            (500,9)
            (1000,9)
    };

==> table/accfeedback.tex <==
\begin{table}
\setlength\extrarowheight{-0.225pt}
\centering
\vspace{0.5em}
\caption{Example Accelerator Relevant Value Spectra}
\label{tab:accfeedback}
\begin{tabular}{lrrrr}
\toprule
Type & \multicolumn{1}{c}{Name} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max}  \\ \hline
input\_value & fpga\_data[size] & 1 & 8 \\
intermediate\_value & i & 0 & 3 \\
intermediate\_value & sum & 0 & 3 \\
mem\_offset & fpga\_data[size] & 0 & 3 \\
loop & SUM\_LOOP & N/A & 2 \\
\bottomrule
\end{tabular}
%\vspace{-3mm}
\end{table}

==> table/executionexample.tex <==
\begin{table*}
\centering
\caption{\bf Example Execution of Five Inputs}\vspace{-2ex}

\label{tab:execution}
\scalebox{0.85}{
\begin{tabular}{clllrrrrrrrrrc}
    \toprule
    \multicolumn{1}{l}{} & \multicolumn{1}{l}{\bf Activated}  
    &\multicolumn{1}{l}{\bf Program} & \multicolumn{1}{l}{\bf Kernel} 
    & \multicolumn{1}{l}{}
    & \multicolumn{4}{c}{\bf FPGA-Relevant Value Spectra} 
    & \multicolumn{1}{l}{\bf New} & \multicolumn{1}{l}{} 
    & \multicolumn{1}{l}{\bf Mutation} & \multicolumn{2}{c}{\bf Memorization}  \\  \cline{6-9}\cline{13-14}
    
    \multicolumn{1}{l}{\bf ID} & \multicolumn{1}{l}{\bf Mutation} &\multicolumn{1}{l}{\bf Inputs} & \multicolumn{1}{l}{\bf Inputs} 
    & \multicolumn{1}{l}{\bf Invoke}
    &\multicolumn{1}{c}{\bf Type} & \multicolumn{1}{c}{\bf Name} & \multicolumn{1}{c}{\bf Min} &  \multicolumn{1}{c}{\bf Max} 
    & \multicolumn{1}{l}{\bf Branch} & \multicolumn{1}{l}{\bf Overflow}
    & \multicolumn{1}{l}{\bf Probability} & \multicolumn{1}{c}{\bf Range} & \multicolumn{1}{c}{\bf Size} \\ \hline
    
    seed & N/A & [1,2,1,2,11] & [1,1,1,9] & yes & input\_value & fpga\_data & 1 & 9 & yes & no & [0.17,0.17,0.17, & (1,9) & 4 \\
    
    {} & {} & {} & {} & {} & variable\_value & i & 0 & 3 & {} & {} & {0.17,0.17,0.17]} & {} & {} \\

    {} & {} & {} & {} & {} & variable\_value & sum & 2 & 12 & {} & {} & {} & {} & {} \\    

    {} & {} & {} & {} & {} & mem\_offset & fpga\_data 
    & \multicolumn{2}{r}{[0,1,2,3]}
    & {} & {} & {} & {} & {} \\   

    {} & {} & {} & {} & {} & loop & SUM\_LOOP & N/A & 2 & {} & {} & {} & {} & {} \\    \hline
    
    1 & M6 & [1,2,1,2,2] & [1,1,1,0] & {\bf no} & N/A & N/A & N/A & N/A & no & N/A & [0.17,0.17,0.17, & (1,9) & 4 \\
    {} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {0.17,0.17,0.17]} & {} & {} \\    \hline
    
    2 & M3 & [1,2,1,2,255] & [1,1,1,253] & yes & input\_value & fpga\_data & {\bf 1} & {\bf 253} & {\bf no} & {\bf yes} & [0.16,0.16,{\bf 0.22}, & {\bf (1,9)} & 4 \\
    
    {} & {} & {} & {} & {} & variable\_value & i & 0 & 3 & {} & {} & {0.16,0.16,0.16]} & {} & {} \\

    {} & {} & {} & {} & {} & variable\_value & sum & {\bf 0} & {\bf 3} & {} & {} & {} & {} & {} \\    

    {} & {} & {} & {} & {} & mem\_offset & fpga\_data 
    & \multicolumn{2}{r}{[0,1,2,3]}
    & {} & {} & {} & {} & {} \\   

    {} & {} & {} & {} & {} & loop & SUM\_LOOP & N/A & 2 & {} & {} & {} & {} & {} \\    \hline
    
    3 & M3 & [0,2,1,2,255] & [2,1,1,253] & yes & input\_value & fpga\_data & 1 & 253 & no & yes & [0.16,0.16,0.22, & (1,9) & 4 \\
    
    {} & {} & {} & {} & {} & variable\_value & i & 0 & 3 & {} & {} & {0.16,0.16,0.16]} & {} & {} \\

    {} & {} & {} & {} & {} & variable\_value & sum & {\bf 1} & {\bf 4} & {} & {} & {} & {} & {} \\    

    {} & {} & {} & {} & {} & mem\_offset & fpga\_data 
    & \multicolumn{2}{r}{[0,1,2,3]}
    & {} & {} & {} & {} & {} \\   

    {} & {} & {} & {} & {} & loop & SUM\_LOOP & N/A & 2 & {} & {} & {} & {} & {} \\ \hline
    
    4 & M1 & [1,2,1,2,11,36] & [1,1,1,9,25] & {\bf yes} & input\_value & fpga\_data & 1 & 25 & no & no & [0.21,0.15,0.21, & (1,25) & 5 \\
    
    {} & {} & {} & {} & {} & variable\_value & i & 0 & 5 & {} & {} & {0.15,0.15,0.15]} & {} & {} \\

    {} & {} & {} & {} & {} & variable\_value & sum & 2 & 37 & {} & {} & {} & {} & {} \\    

    {} & {} & {} & {} & {} & mem\_offset & fpga\_data 
    & \multicolumn{2}{r}{[0,1,2,3,4,5]}
    & {} & {} & {} & {} & {} \\   

    {} & {} & {} & {} & {} & loop & SUM\_LOOP & N/A & 3 & {} & {} & {} & {} & {} \\    

    \bottomrule
    \end{tabular}
}
\vspace{-2ex}
\end{table*}

==> table/pragma.tex <==
\begin{table*}
\centering
\caption{\bf Mapping from HLS Pragmas to Hardware Value Spectra}\vspace{-2ex}
\label{tab:pragma}
\scalebox{0.85}{
\begin{tabular}{p{1.5cm}|l|l|l}
\toprule
{} & {} & {}& \textbf{FPGA-Relevant} \\ 

{\bf Category} & {\bf HLS Directive /Pragma} & {\bf Description of Pragma} & \textbf{Value Spectra} \\ \hline

{Data Type} & \codefont{typedef ap\_uint$<$x$>$ bitx} & {Define an unsigned Integer with a custom bitwidth} & {The actual variable values with this type} \\ \cline{2-3}
{} & \codefont{typedef ap\_int$<$x$>$ bitx} & {Define a signed Integer with a custom bitwidth} & {}\\ \hline

{} & \codefont{\#pragma HLS array\_partition} & {Partition an array into smaller arrays or individual elements} & \\ \cline{2-3}
{Memory} & \codefont{\#pragma HLS array\_reshape} & {Combine array partitioning with vertical array mapping}  & {The set of accessed offsets} \\ \cline{2-3}
{} & \codefont{\#define size M} & {Defines the estimated array size} & {} \\ \hline

{Recursion} & N/A & N/A & The actual used size of\\ 
& & & stack and the number of iterations \\\hline

{Parallelization} & \codefont{\#pragma HLS dataflow} & Enable task-level pipelining & The fifo queue size \\\cline{2-3}
{} & \codefont{\#pragma HLS pipeline} & Allow concurrent execution of operations &{if feedback path exists  } \\\hline

{} & \codefont{\#pragma HLS unroll}& Creat multiples copies of the loop body &  \\ \cline{2-3}
{Loop} & \codefont{\#pragma HLS loop\_tripcount} & {Specifie the total number of iterations} & {The actual number of iterations}\\ \cline{2-3}
{} & \codefont{\#pragma HLS loop\_flatten} & {Allow nested loops to be flattened into a single loop hierarchy} & {} \\ \cline{2-3}
{} & \codefont{\#pragma HLS loop\_merge} & {Merge consecutive loops into a single loop to reduce overall latency} & {}\\ \hline

{Interface/} & \codefont{\#pragma HLS INTERFACE} & {Perform input and output operations using a specific I/O protocol} & {N/A} \\
{Configuration} & {etc.} & {in the design interface} & {}\\
\bottomrule
\end{tabular}
}
\vspace{-2ex}
\end{table*}

==> table/subjects.tex <==
\begin{table*}[t]
    \centering    \caption{Subject Programs}
    \scalebox{0.9}{
    \begin{tabular}{clllcp{1.1cm}<{\centering}p{0.8cm}<{\centering}p{1.1cm}<{\centering}p{0.8cm}<{\centering}}
    \toprule
        {}&{}&{}&{}&{}&\multicolumn{2}{c}{\bf \# of Detected}&\multicolumn{2}{c}{\bf \% of Div-inducing } \\
        {} & {\bf Subject} & {} & {} & {\bf \# of} & \multicolumn{2}{c}{\bf Symptoms} &\multicolumn{2}{c}{\bf Inputs}  \\\cline{6-7}\cline{8-9}
        {\bf ID} & {\bf Program} & {\bf Kernel} & {\bf Description} & {\bf Pragmas} & {\bf HeteroFuzz} & {\bf \randomfuzzS}&{\bf HeteroFuzz} &{\bf  \randomfuzzS} \\\hline
        P1 & Median Filter & Bubble Sort & Blur an image by replacing the pixel value to a median & 10 & 6 & 1 & 68.2\% & 6.8\%\\
        P2 & Median Filter & Merge Sort & Blur an image by replacing the pixel value to a median & 8 & 6 & 1 & 37.3\% & 4.5\% \\
        P3 & Image Denoising & Accumulation & {Denoise an image based on analyzing image gradients} & 10 & 5 & 0 & 71.0\% & 0\%\\
        P4 & KNN & L2norm & Finds the top-k most relevant elements & 12 & 5 & 2 & 72.9\% & 14.5\% \\
        P5 & Signal Transmission & RGB2YUV & Transform RGB signals to YUV signals & 15 & 7 & 2 & 40.0\% & 4.5\% \\
        P6 & 3D Rendering & Rendering & Render an image based on 3D information & 12 & 9 & 2 & 56.0\% & 10.0\%\\
        P7 & Face Detection & Detection & {Detect human faces in an image} & 17 & 9 & 2 & 52.2\% & 5.0\% \\

    \bottomrule
    \end{tabular}
    }
    \label{tab:subjects}
    \vspace{-2ex}
\end{table*}

==> table/symptom.tex <==
\begin{table}[t]
    \centering    \caption{Example Divergence Symptoms for P3}
    \scalebox{0.95}{
    \begin{tabular}{cll}
    \toprule
        {\bf ID} & {\bf Symptom} & {\bf Example}\\ \hline
        S1 & Unexpected Endless Loop & {Memory overflow happens when  }\\
        & & FPGA attempts to write \\
        & & {\codefont{data\_fpga} at an unexpected}\\
        & & address in line 27 of Figure~\ref{fig:accumulationC}.\\\hline
        S2 & Kernel Offloading Error & {Host is offloading a large number  }\\
        & & 2147483600 to FPGA \\
        & & in line 27 of Figure~\ref{fig:accumulationC}, leading\\
        & & to a wrong returned result.\\\hline
        S3 & Kernel Runtime Overflow & {The value of intermediate variables } \\
        & & in line 32 of Figure~\ref{fig:accumulationC} \\
        & & exceeds its bitwidth capacity, \\
        & & leading to a wrong returned result.\\\hline
        S4 & Divide by Zero in Host & {FPGA returned result leads to }\\
        & & divide-by-zero error\\
        & &  in line 10 of Figure~\ref{fig:motivating}.\\\hline
        S5 & Incorrect Loop Unrolling & {CPU and FPGA produce different }  \\
        & & results for Figure~\ref{fig:motivating} when the input\\
        & & array size is not multiple of 2.\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:symptom}
    \vspace{-2ex}
\end{table}
